FLEX: Feature-Logic Embedding Framework for CompleX Knowledge Graph Reasoning

Current best performing models for knowledge graph reasoning (KGR) introduce geometry objects or probabilistic distributions to embed entities and first-order logical (FOL) queries into low-dimensional vector spaces. They can be summarized as a center-size framework (point/box/cone, Beta/Gaussian distribution, etc.). However, they have limited logical reasoning ability. And it is difficult to generalize to various features, because the center and size are one-to-one constrained, unable to have multiple centers or sizes. To address these challenges, we instead propose a novel KGR framework named Feature-Logic Embedding framework, FLEX, which is the first KGR framework that can not only TRULY handle all FOL operations including conjunction, disjunction, negation and so on, but also support various feature spaces. Specifically, the logic part of feature-logic framework is based on vector logic, which naturally models all FOL operations. Experiments demonstrate that FLEX significantly outperforms existing state-of-the-art methods on benchmark datasets.

==> paper_section/010_introduction_2cols.tex <==
% TODO **贡献**
% ! 1. 据我们所知，这是第一个**真正意义上具有完整的逻辑建模能力的KGE模型**。
% ? 2. 提出一个灵活的CQE框架，查询表示被解耦为**特征表示部分**和**逻辑表示部分**。这意味着对于包括Transformer、CNN、GNN在内的所有模型给出的特征表示，只需简单地加上逻辑表示部分，即可构建一个具有逻辑表示能力的模型。
% ? 3. 本文提供两种可选的逻辑表示，向量逻辑和量子逻辑，具有良好的数学性质和物理意义，为下游任务提供多样的选择。
% ? 4. 本文实验完善，实验结果超过SOTA。

% Knowledge graphs (KGs) stores real-world knowledge or facts in a directed graph.
One of the fundamental tasks in knowledge graphs (KGs) is knowledge graph reasoning (KGR), which aims to infer new facts by performing complex multi-hop logical reasoning over the given KG.
Since the KGs are usually large and incomplete, the KGR task is challenging.
In general, multi-hop logical reasoning answers a first-order logic (FOL) query involving logical and relational operators.
Recently, the most popular models for logical reasoning are embedding-based.
These methods represent the query as low-dimensional embedding, which are used to rank against all candidate entities to find the answers.
Figure~\ref{fig:query} shows a multi-hop query example and its computation graph.

Current common embedding-based methods include:
(1) distribution-based model such as: BetaE~\cite{BetaE} and PERM~\cite{PERM},
(2) geometry-based model such as Q2B~\cite{Query2box}, ConE~\cite{ConE}, HypE~\cite{HypE}.
These methods can be characterized as a center-size framework, where the center parameter represents semantic position and the size parameter represents boundary.
For example, in PERM, center is the mean value and size is covariance value of the Gaussian distribution.
In Q2B, center is the center of box, while size is the offset of the box.
In ConE, center is the axis and size is the aperture.

\begin{figure*}
    \centering
    % \vspace{-3mm}
    \includegraphics[width=0.8\textwidth]{query3.drawio.png}
    \caption{A multi-hop logical query and its computation graph.}
    \vspace{-3mm}
    \label{fig:query}
\end{figure*}

% Queries involving all FOLs are ubiquitous in real world application.

% However, we notice two issues in center-size framework.
% First, \textbf{the logical operations are not all closed in center-size framework}.
% For example, it is infeasible to use Beta distribution to represent Difference operation, because the difference of Beta distributions is not a Beta distribution.
% Besides, if center-size framework accurately models any Existential Positive First-order (EPFO) logical queries, the dimensionality of the logical query embeddings needs to be $\mathcal{O}(|\mathcal{V}|)$~\cite{Query2box}, where $|\mathcal{V}|$ is the count of all entities, not low-dimensional anymore.
% The low-level object and embedding dimension are key limitations to prevent center-size framework from keeping all logical operations closed.
% Secondly, \textbf{the feature description and logical representation are coupled in center-size framework, hard to generalize to new features}.
% In real world KGs, the features of entities are usually heterogeneous, such as text, image, and graph.
% These features contribute to reasoning, so a good reasoning framework should consider the extension to integrate new features.
% However, current center-size framework has a one-to-one constraint on center and size, which restricts the extensibility and flexibility of the model.
% For example, ConE requires that one axis must correspond to one aperture, to represent sector-cone.
% Appending new feature will result in second axis.
% But it's difficult for ConE to generalize to the case where two axes correspond to one aperture, because this case is not a valid parameterization of sector-cone.

However, we have identified two issues with the center-size framework.
First, \textbf{not all logical operations are closed under this framework}.
For example, it is not possible to use the Beta distribution to represent the difference operation, because the difference of two Beta distributions is not a Beta distribution.
Additionally, if the center-size framework can accurately model Existential Positive First-order (EPFO) logical queries, the dimensionality of the logical query embeddings would need to be $\mathcal{O}(|\mathcal{V}|)$~\cite{Query2box}, where $|\mathcal{V}|$ is the number of entities, which is not low-dimensional.
The low-level object and high-dimensional embedding are key limitations that prevent the center-size framework from being able to represent all logical operations.
Secondly, \textbf{the coupling of feature description and logical representation in the center-size framework makes it difficult to generalize to new features.}.
In real world KGs, the features of entities are usually heterogeneous, such as text, image, and graph.
These features contribute to reasoning, so a good reasoning framework should consider the extension to integrate new features.
However, the current center-size framework has a one-to-one constraint on the center and size, which limits the extensibility and flexibility of the model.
For example, ConE requires that one axis must correspond to one aperture, to represent sector-cone.
Adding a new feature would require a second axis, but it would be difficult for ConE to generalize to the case where two axes correspond to one aperture, because this would not be a valid parameterization of a sector-cone.
% Appending new feature will result in second axis.
% But it's difficult for ConE to generalize to the case where two axes correspond to one aperture, because this case is not a valid parameterization of sector-cone.

% We have identified two issues with the center-size framework.
% First, not all logical operations are closed under this framework.
% For example, it is not possible to use the Beta distribution to represent the difference operation, because the difference of two Beta distributions is not a Beta distribution.
% Additionally, if the center-size framework can accurately model existential positive first-order (EPFO) logical queries, the dimensionality of the logical query embeddings would need to be $\mathcal{O}(|\mathcal{V}|)$, where $|\mathcal{V}|$ is the number of entities, which is not low-dimensional.
% The low-level object and high-dimensional embedding are key limitations that prevent the center-size framework from being able to represent all logical operations.
% Second, the feature description and logical representation are coupled in the center-size framework, making it difficult to generalize to new features.
% In real-world knowledge graphs, the features of entities are often heterogeneous, such as text, images, and graphs.
% These features are important for reasoning, so a good reasoning framework should be able to integrate new features.
% However, the current center-size framework has a one-to-one constraint on the center and size, which limits the extensibility and flexibility of the model.
% For example, ConE requires that one axis must correspond to one aperture in order to represent a sector-cone.
% Adding a new feature would require a second axis, but it would be difficult for ConE to generalize to the case where two axes correspond to one aperture, because this would not be a valid parameterization of a sector-cone.
%  The representation ability of distributions or geometric objects is limited by its low-level object and embedding dimension.
% The only solution is to increase embedding dimension of the sector-cones, which will result in simultaneous increase in the parameters of centers and sizes.

Therefore, it is of great significance to propose a new embedding-based framework that (1) keeps closed under all logical operations and (2) is easy to generalize to new features.
We consider dividing the embeddings of entities and queries into two loosely coupled parts, feature part and logic part, and then learns each part independently.
In this way, we can easily extend the model to new features (by adding new feature parts) and keep all logical operations closed (by introducing closed fuzzy logic).
% One part is responsible for feature description, and the other part is for logic representation.
For the feature parts, neural networks are adopted to capture the query representation and logical information.
For the logic parts, we propose to use \textbf{vector logic} to guarantee to model at least all logical operators, directly.
We use vector logic because it is a fuzzy logic system based on matrix algebra, easy to cope with neural networks.
% Recent papers use t-norm (CQD~\cite{CQD}), distribution (BetaE~\cite{BetaE}) or geometric object (Query2box~\cite{Query2box}, ConE~\cite{ConE}) to simulate logical computing including AND, OR, NOT, without the consideration of other logic operations like exclusive or(XOR), implication(IMPL), etc.
% By contrast, vector logic considers all logical operations, promoting our framework to build all closed neural logical operators.

Feature-Logic framework has the following advantages:
(1) \xhdr{All neural logical operators are closed}
The FOL operations include conjunction, disjunction, negation, etc.
These operations on feature-logic embeddings generate feature-logic embedding, which means that all neural operators are closed.
Furthermore, we also prove that these operators based on feature-logic embedding obey the rules of real logical operations in Section~\ref{sec:model:theoretical_analysis}.
% The logic part, which represents the logical state, is used to integrate the logical reasoning ability into the plain feature embedding.
% In this paper, vector logic which can handle all FOL operations is adopted as the logic part.
% In this way, our framework possess comprehensive logical reasoning capability.
(2) \xhdr{High extensibility and flexibility}
Unlike centers-size framework, our framework has fewer constraints on each part.
On the one hand, feature-logic embedding can extend to multiple independent feature parts, which help to integrate heterogeneous information as a result of more precise description of entities in KGs.
The feature part is also able to choose a variety of feature spaces, such as limited or infinite real space (and complex space, theoretically).
On the other hand, the logic part can be modified without impacting on the feature part.
It is also allowed to replace vector logic with other fuzzy system on the logic part.
% The logic states before and after calculation do not depend on the feature part.
% Instead, the feature part depends on the logic part to capture the hidden information in logical transformation.

We summarized our contributions as follows:
(1) We propose a closed embedding-based framework FLEX for knowledge graph reasoning, which not only supports various feature spaces, but also has all closed logical operators, including conjunction, disjunction, negation, etc.
(2) To our best knowledge, we are the first to introduce vector logic into the field of logical reasoning over knowledge graphs.
(3) Experiments on benchmark datasets demonstrate that our framework significantly outperforms state-of-the-art models. The source code is also available online (Appendix~\ref{sec:appendix:train}).


==> paper_section/030_preliminary.tex <==
% ? 1. 背景知识
% ?     1. 知识图谱
% ?     2. 一阶逻辑
% ?     3. 计算图
% ?     4. 查询嵌入表示
% ? 2. 向量逻辑的**定义**和**一般结论**（与或非等公式）
% ? 3. 量子逻辑的**定义**和**一般结论**（与或非等公式）
% ? 1a-1d参考ConE论文，2参考[https://zh.wikipedia.org/wiki/向量邏輯](https://zh.wikipedia.org/wiki/%E5%90%91%E9%87%8F%E9%82%8F%E8%BC%AF) ，3参考[https://zh.wikipedia.org/wiki/量子位元](https://zh.wikipedia.org/wiki/%E9%87%8F%E5%AD%90%E4%BD%8D%E5%85%83)
% ? 向量逻辑部分需要包括这些公式（量子逻辑部分模仿向量逻辑部分给出类似的公式）
% \subsection{Backgrounds of Embedding-based Methods}
\xhdr{Knowledge Graph (KG)}
A knowledge graph $G = \{\mathcal{V}, \mathcal{R}, \mathcal{T}\}$ consists of entity set $\mathcal{V}$, relation set $\mathcal{R}$ and triple set $\mathcal{T} = \{(h, r, t)| h, t\in \mathcal{V}; r\in \mathcal{R}\}$, where $h$, $r$ and $t$ denotes head entity, relation and tail entity respectively.

\xhdr{First-Order Logical (FOL) Query}
A FOL query $q$ consists of a non-variable anchor entity set $V_a \subseteq \mathcal{V}$, existentially quantified bound variables $V_1, V_2, \cdots, V_k$, target variable $V_?$, relation $r \in \mathcal{R}$ in the KG and logical operations existential quantification $\exists$, monadic operators (identity, negation $\neg$) and dyadic operators (conjunction $\cap$, disjunction $\cup$, implication $\text{IMPL}$, equivalence $E$, exclusive or $\text{XOR}$, etc.).
The \underline{d}isjunctive \underline{n}ormal \underline{f}orm (DNF) of a query $q$ is defined as:
\begin{equation}
  q[V_?] = V_?, \exists V_1, \cdots, V_k:c_1 \lor c_2 \lor \cdots \lor c_n
\end{equation}
where $c_i$ represents conjunctions of one or more literals $e$, \ie, $c_i = e_{i1} \land e_{i2} \land \cdots \land e_{im}$ and literal $e$ represents an atomic formula or its negation, \ie, $e_{ij} = r(v_a, V)$ or $\lnot r(v_a, V)$ or $r(V', V)$ or $\lnot r(V', V)$, where $v_a \in V_a, V \in \{V_?, V_1, V_2, \cdots, V_k\}, V'\in \{ V_1, V_2, \cdots, V_k\}$ and $V \ne V'$.

\xhdr{Computation Graph}
A computation graph is a directed acyclic graph whose nodes represent entity sets $V_a \cup V$ in the query structure, while directed edges represent logical or relational operations acting on the entity sets.
% A computation graph specifies how the reasoning of the query is proceeded on KGs.
Starting from anchor entity sets, we obtain the answer entity set after applying operations on the entity sets according to the directed edges in the computation graph.
The operation types on the computation graph are defined as follows:
(1) \textbf{Relational Projection $\mathcal{P}$}: Given an entity set $S \subseteq \mathcal{V}$ and a relation $r \in \mathcal{R}$, project operation maps $S$ to another entity set $S'=\cup_{v\in S}\{v'|(v, r,v')\in\mathcal{T}\}$.
(2) \textbf{Monadic Operators}: \textbf{Identity} and \textbf{Complement/Negation} $\mathcal{C}$. The complement set of given entity set $S$ in KG is $\bar{S} = \mathcal{V} \backslash S$.
(3) \textbf{Dyadic Operators}: \textbf{Intersection} $\mathcal{I}$, \textbf{Union} $\mathcal{U}$, \textbf{Implication} $\text{IMPL}$, \textbf{Equivalence} $E$, \textbf{Exclusive-or} $\text{XOR}$, etc. Given a set of entity sets $\{S_1, \cdots, S_n\}$, the intersection (union, etc.) operation computes logical intersection (union, etc.) of these sets $\cap_{i=1}^nS_i$ ($\cup_{i=1}^nS_i$, etc.).

\xhdr{Query Embedding}
A query embedding $\mathbf{V}_q$ of query set $q$ is a continuous embedding.
Starting from anchor entity sets, we obtain the final embedding $\mathbf{V}_q$ for query $q$ after applying operations according to computation graph.
The answer to the query $q$ is the entities $v$ whose embedding $\mathbf{v}$ has the smallest distance $dist(\mathbf{v}, \mathbf{V}_q)$ to the embedding of query $q$.

% \subsection{Quantum Logic}

% A knowledge graph can be represented as $KG=\{E, R, A, V, T^R, T^A\}$, where $E$ is the set of entities, $R$ is the set of relations, $A$ is the set of attributes, $V$ is the set of attribute values, $T^R=\{ (h,r,t) \in E \times R \times E \}$ is the set of relation triples, and $T^A=\{ (e,a,v) \in E \times A \times V \}$ is the set of attribute triples. Relation triple $(h,r,t)$ consists of head entity $h \in E$, relation $r \in R$ and tail entity $t \in E$. Attribute triple $(e,a,v)$ consists of entity $e \in E$, attribute $a \in A$ and attribute value $v \in V$.

% Given $KG_1=\{E_1, R_1, A_1, V_1, T^R_1, T^A_1\}$, $KG_2=\{E_2, R_2, A_2, V_2, T^R_2, T^A_2\}$ and pre-aligned seeds $P_{\text{seed}}=\{(e_{1}, e_{2}) \in E^{\text{seed}}_{1} \times E^{\text{seed}}_{2}, e_1 \leftrightarrow e_2\}$ where $\leftrightarrow$ represents equivalence, $|P_{\text{seed}}| = |E^{\text{seed}}_1| = |E^{\text{seed}}_2|$ and $E^{\text{seed}}_i \subseteq E_i (i=1,2)$, we split pre-aligned seeds to training set $P_{\text{train}}=\{(e_{1}, e_{2}) \in E^{\text{train}}_{1} \times E^{\text{train}}_{2}, e_1 \leftrightarrow e_2\}$ and testing set $P_{\text{test}}=\{(e_{1}, e_{2}) \in E^{\text{test}}_{1} \times E^{\text{test}}_{2}, e_1 \leftrightarrow e_2\}$ where $P_{\text{train}} \cap P_{\text{test}} = \emptyset$,$P_{\text{train}} \cup P_{\text{test}} = P_{\text{seed}}$. EA task is to predict $? \in E^{\text{test}}_{2}$ for $(e_{1}, ?)$ given $e_1 \in E^{\text{test}}_{1}$ (left-to-right prediction) and $? \in E^{\text{test}}_{1}$ for $(?,e_{2})$ given $e_2 \in E^{\text{test}}_{2}$(right-to-left prediction). A bootstrapping strategy is to generate likely entity pairs $P'=\{(e_{1}, e_{2}) \in E^{\text{test}}_{1} \times E^{\text{test}}_{2}\}$ to expand training set $P_{\text{train}}$. For $(e_1,e_2)$ in $P'$, equivalence may not hold between $e_1$ and $e_2$.



==> paper_section/040_model_2cols.tex <==
In this section, we propose feature-logic embedding framework (FLEX) for KGR.
We first introduce how to reason using first-order logic in Section~\ref{sec:model:common} and vector logic in Section~\ref{sec:model:vector_logic}
%  and components of feature-logic embeddings for queries and entities in Section~\ref{sec:model:component}.
Afterwards, we present feature-logic embeddings and the methods to learn in Section~\ref{sec:model:component}, \ref{sec:model:operators} and \ref{sec:model:learn_embedding}.
Furthermore, we provide theoretical analysis in Section~\ref{sec:model:theoretical_analysis} to show that FLEX is closed, and obeys the rules of real logical operations.

\subsection{First-Order Logic for Knowledge Graph}
\label{sec:model:common}

\xhdr{Knowledge Graph} $\mathcal{G} = \{\mathcal{V}, \mathcal{R}, \mathcal{T}\}$ consists of entity set $\mathcal{V}$, relation set $\mathcal{R}$ and triple set $\mathcal{T} = \{(h, r, t)| h, t\in \mathcal{V}; r\in \mathcal{R}\}$, where $h$, $r$ and $t$ denotes head entity, relation and tail entity respectively.
% Because KGs are large and incomplete, classical boolean logic is not appliable to infer all answers for given queries.
% We need to adjust the logic to handle the incompleteness of KGs.

\xhdr{First-Order Logic (FOL)} In the query embedding literature, FOL queries typically involve logical operations such as existential quantification ($\exists$), monadic operations (identity, negation $\neg$) and dyadic operations (conjunction $\cap$, disjunction $\cup$, implication $\rightarrow $, equivalence $\leftrightarrow $, exclusive or $\oplus$, etc.). However, universal quantification ($\forall$) is not typically included, as it is not typically applicable in real-world knowledge graphs where no entity connects with all other entities~\cite{Query2box,BetaE,ConE}.

% \xhdr{First-Order Logic (FOL)} FOL query $q$ involves relational projection $r \in \mathcal{R}$ and logical operations including existential quantification $\exists$, monadic operators (identity, negation $\neg$) and dyadic operators (conjunction $\cap$, disjunction $\cup$, implication $\rightarrow $, equivalence $\leftrightarrow $, exclusive or $\oplus$, etc.).
% Universal quantification ($\forall$) is not considered, because no entity connects to all entities in real-world KGs~\cite{Query2box,BetaE,ConE}.
%  a non-variable anchor entity set $V_a \subseteq \mathcal{V}$, existentially quantified bound variables $V_1, V_2, \cdots, V_k$, target variable $V_?$,

To formulate FOL query $q$, we use its \underline{d}isjunctive \underline{n}ormal \underline{f}orm (DNF)\cite{Query2box} which is defined as:
\begin{equation}
  q = V_?, \exists V_1, \cdots, V_k:c_1 \lor c_2 \lor \cdots \lor c_n
\end{equation}
where $V_?$ is target variable, $V_1, \cdots, V_k$ are existentially quantified bound variables, $c_i$ represents conjunctions, \ie, $c_i = e_{i1} \land e_{i2} \land \cdots \land e_{im}$ and literal $e$ represents an atomic formula or its negation, \ie, $e_{ij} = \mathcal{P}_{r}(v_a, V)$ or $\lnot \mathcal{P}_{r}(v_a, V)$ or $\mathcal{P}_{r}(V', V)$ or $\lnot \mathcal{P}_{r}(V', V)$, where $v_a \in V_a \subseteq \mathcal{V}$ is a non-variable anchor entity set, $V \in \{V_?, V_1, \cdots, V_k\}$, $V'\in \{ V_1, \cdots, V_k\}$ and $V \ne V'$, $\mathcal{P}_{r} : \mathcal{V} \times \mathcal{V} \to \{\text{True}, \text{False}\}$ is the predicate corresponding to relation $r\in\mathcal{R}$. $\mathcal{P}_{r}(V_h, V_t)=\text{True}$ if and only if $(h, r, t)$ is a factual triple in $\mathcal{T}$, $\forall h \in V_h \subseteq \mathcal{V}, t\in V_t \subseteq \mathcal{V}$.
Answering query $q$ is to find the entity set $\llbracket q\rrbracket \subset \mathcal{V}$, where $v\in\llbracket q\rrbracket$ if and only if $q[v]$ is true.

% The \underline{d}isjunctive \underline{n}ormal \underline{f}orm (DNF) of query $q$ is defined as:
% \begin{equation}
%   q[V_?] = V_?, \exists V_1, \cdots, V_k:c_1 \lor c_2 \lor \cdots \lor c_n
% \end{equation}
% where $c_i$ represents conjunctions of one or more literals $e$, \ie, $c_i = e_{i1} \land e_{i2} \land \cdots \land e_{im}$ and literal $e$ represents an atomic formula or its negation, \ie, $e_{ij} = r(v_a, V)$ or $\lnot r(v_a, V)$ or $r(V', V)$ or $\lnot r(V', V)$, where $v_a \in V_a, V \in \{V_?, V_1, V_2, \cdots, V_k\}, V'\in \{ V_1, V_2, \cdots, V_k\}$ and $V \ne V'$.

\xhdr{Computation Graph}
The reasoning procedure for FOL query can be represented as a computation graph (Figure~\ref{fig:query}), where nodes represent entity sets and edges represent logical operations.
To make the computation work in embedding space, query embedding methods generate low-dimensional embeddings for nodes and map edges to logical operators as follows:

\textbf{Projection Operator $\mathcal{P}$}: Given an entity set $S \subseteq \mathcal{V}$ and a relation $r \in \mathcal{R}$, project operation maps $S$ to tail entity set $S'=\cup_{v\in S}\{v'|(v, r,v')\in\mathcal{T}\}$.

\textbf{Monadic Operators}: \textbf{Identity} and \textbf{Negation} $\mathcal{N}$. The complement set of given entity set $S$ in KG is $\bar{S} = \mathcal{V} \backslash S$.

\textbf{Dyadic Operators}: \textbf{Intersection} $\mathcal{I}$, \textbf{Union} $\mathcal{U}$, \textbf{Implication} $\mathcal{L}$, \textbf{Exclusive-or} $\mathcal{X}$, etc. Given a set of entity sets $\{S_1, \cdots, S_n\}$, the intersection (union, etc.) operation computes logical intersection (union, etc.) of these sets $\cap_{i=1}^n S_i$ ($\cup_{i=1}^n S_i$, etc.).


% A computation graph is a directed acyclic graph whose nodes represent entity sets $V_a \cup V$ in the query structure, while directed edges represent logical or relational operations acting on the entity sets.
% A computation graph specifies how the reasoning of the query is proceeded on KGs.
% Starting from anchor entity sets, we obtain the answer entity set after applying operations on the entity sets according to the directed edges in the computation graph.
% The operation types on the computation graph are defined as follows:

% \xhdr{Query Embedding}
% A query embedding $\mathbf{V}_q$ of query set $q$ is a continuous embedding.
% Starting from anchor entity sets, we obtain the final embedding $\mathbf{V}_q$ for query $q$ after applying operations according to computation graph.
% The answer to the query $q$ is the entities $v$ whose embedding $\mathbf{v}$ has the smallest distance $dist(\mathbf{v}, \mathbf{V}_q)$ to the embedding of query $q$.

\subsection{Vector Logic}
\label{sec:model:vector_logic}

We follow the definition of vector logic in \cite{vector_logic}. Vector logic is an elementary logical model based on matrix algebra.
In vector logic, true value are mapped to the vector, and logical operators are executed by matrix computation.

\xhdr{Truth Value Vector Space}
A two-valued vector logic use two $d$-dimensional ($d \ge 2$) column vectors $\vec{s}$ and $\vec{n}$ to represent true and false in the classic binary logic.
$\vec{s}$ and $\vec{n}$ are real-valued, normally orthogonal to each other, and normalized vectors, \ie, $\|\vec{s}\|=1, \|\vec{n}\|=1, \vec{s}^T\vec{u}=0$.
% Truth value vector space are generated by $V_2 = \{\vec{s}, \vec{n}\}$, and operations on vectors in truth value space is based on scalar product.

\xhdr{Operators}
The basic logical operators are associated with its own matrices by vectors in truth value vector space.
Two common types of operators are monadic and dyadic.

(1) Monadic Operators:
Monadic operators are functions: $\mathbb{V} \to \mathbb{V}$.
Two examples are Identity $I = \vec{s} \vec{s}^T + \vec{n} \vec{n}^T$ and Negation $N = \vec{n} \vec{s}^T + \vec{s} \vec{n}^T$ such that $I\vec{s} = \vec{s}, I\vec{n} = \vec{n}, N\vec{n} = \vec{s}, N\vec{s} = \vec{n}$.

(2) Dyadic Operators:
Dyadic operators are functions: $\mathbb{V} \otimes \mathbb{V} \to \mathbb{V}$, where $\otimes$ denotes Kronecker product.
Dyadic operators include conjunction $C$, disjunction $D$, implication $L$, exclusive or $X$, etc.
For example, the conjunction between two logical propositions $(p\land q)$ is performed by $C(\vec{u}\otimes \vec{v})$, where $C=\vec{s}(\vec{s} \otimes \vec{s})^T+\vec{n}(\vec{s} \otimes \vec{n})^T+\vec{n}(\vec{n} \otimes \vec{s})^T+\vec{n}(\vec{n} \otimes \vec{n})^T$.
It can be verified that $C(\vec{s} \otimes \vec{s})=\vec{s},C(\vec{s} \otimes \vec{n}) = C(\vec{n} \otimes \vec{s}) = C(\vec{n} \otimes \vec{n}) = \vec{n}$.
% Dyadic operators which correspond to logical operations in classic binary logic are defined by its formulation to perform logical operations on truth value vectors.
% Their associated matrices has $d^2$ rows and $d$ columns.

\xhdr{Many-valued Two-dimensional Logic}
Many-valued logic are introduced to include uncertainties in the logic vector.
Weighting $\vec{s}$ and $\vec{n}$ by probabilities, uncertainties are introduced: $\vec f = \epsilon \vec{s} + (1-\epsilon) \vec{n}$, where $\epsilon \in [0,1]$.
Besides, operations on vectors can be simplified to computation on the scalar of these vectors.
For example, given two vectors $\vec{u} = \alpha \vec{s} + (1-\alpha) \vec{n}, \vec{v}= \alpha' \vec{s} + (1-\alpha') \vec{n}$, we have:
\begin{equation*}\label{eq:vector_logic}
  \begin{aligned}
    \text{NOT}(\alpha)           & =\vec{s}^T N\vec{u} = 1 - \alpha                                    \\
    \text{OR}(\alpha, \alpha')   & =\vec{s}^T D(\vec{u} \otimes \vec{v})=\alpha+\alpha'-\alpha\alpha'  \\
    \text{AND}(\alpha, \alpha')  & =\vec{s}^T C(\vec{u} \otimes \vec{v})=\alpha\alpha'                 \\
    \text{IMPL}(\alpha, \alpha') & =\vec{s}^T L(\vec{u} \otimes \vec{v})=1-\alpha(1-\alpha')           \\
    \text{XOR}(\alpha, \alpha')  & =\vec{s}^T X(\vec{u} \otimes \vec{v})=\alpha+\alpha'-2\alpha\alpha'
  \end{aligned}
\end{equation*}

\subsection{Feature-Logic Embeddings for Queries and Entities}
\label{sec:model:component}
% In general, the answer entities to a query $q$ have similar semantics under the context of query $q$.
% So when we embed an entity query set $\llbracket q\rrbracket$ into an embedding space, we expect entities $v\in\llbracket q\rrbracket$ to have similar embeddings.
% We design a distance function to measure the similarity between the query embedding and the entity embedding.
% In this way, if the similarity score is high, then the entity is likely to be an answer.

In this section, we design embeddings for queries and entities.
To model the logical information hidden in the query embedding, we propose to consider a part of the embedding as logic part, while the rest as feature part.
The logic part obeys the rules of real logical operations in vector logic and doesn't depend on the feature part.
Formally, the embedding of $\llbracket q\rrbracket$ is $\mathbf{V}_q=(\boldsymbol{\theta}_{f}, \boldsymbol{\theta}_{l})$ where $\boldsymbol{\theta}_{f}\in [-L,L]^d$ is the feature part and $\boldsymbol{\theta}_{l} \in [0,1]^d$ is the logic part, $d$ is the embedding dimension and $L>0$ is a boundary.
In vector logic, the parameter $\boldsymbol{\theta}_{l}$ is the uncertainty $\boldsymbol{\theta}_{l}\vec{s} + (1-\boldsymbol{\theta}_{l})\vec{n}$ of the feature.

An entity $v\in\mathcal{V}$ is a special query without uncertainty.
We propose to represent an entity as the query with logic part $\boldsymbol{0}$, which indicates that the entity's uncertainty is $0$. Formally, the embedding of entity $v$ is $\textbf{v}=(\boldsymbol{\theta}_{f}, \boldsymbol{0})$, where $\boldsymbol{\theta}_{f}\in [-L,L]^d$ is the feature part and $\boldsymbol{0}$ is a $d$-dimensional vector with all elements being 0.

\subsection{Logical Operators for Feature-Logic Embeddings}
\label{sec:model:operators}

\begin{figure*}[t]
  \vspace{-1mm}
  \centering
  \begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=\textwidth]{projection.png}
    \vspace{-5mm}
    \caption{Projection}
    \label{subfig:projection}
  \end{subfigure}\hfil
  \begin{subfigure}[b]{0.23\textwidth}
    \includegraphics[width=\textwidth]{complement.png}
    \vspace{-5mm}
    \caption{Negation}
    \label{subfig:complement}
  \end{subfigure}\hfil
  \begin{subfigure}[b]{0.265\textwidth}
    \includegraphics[width=\textwidth]{intersection.png}
    \vspace{-5mm}
    \caption{Intersection}
    \label{subfig:intersection}
  \end{subfigure}\hfil
  \begin{subfigure}[b]{0.265\textwidth}
    \includegraphics[width=\textwidth]{union.png}
    \vspace{-5mm}
    \caption{Union}
    \label{subfig:union}
  \end{subfigure}\hfil
  \vskip -1mm
  \caption{FLEX's neural logical operators. Each query embedding consists of feature part and logic part. The feature part depends on previous feature and logic parts. The logic part obeys the rules of real logical operations independently.}
  \label{fig:models}
  \vspace{-4mm}
\end{figure*}

In this section, we introduce the designed logical operators, including projection, intersection, complement, union, and other dyadic operators.
% Note that our feature-logic framework is able to directly model all dyadic operators, which is different from center-size framework.

% In addition, we use the vector logic introduced in Section~\ref{sec:model:vector_logic}.
% The logic part of our framework can be replaced with other continuous logic.

\xhdr{Projection Operator $\mathcal{P}$}
The goal of operator $\mathcal{P}$ is to map an entity set to another entity set under a given relation. We define a function $f_r : \mathbf{V}_q \mapsto \mathbf{V}_q'$ in the embedding space to represent $\mathcal{P}$. To implement $f_r$, we first represent relations as translations on query embeddings and assign each relation with relational embedding $\mathbf{r}=(\boldsymbol{\theta}_{f,r}, \boldsymbol{\theta}_{l,r})$. Then $f_r$ is defined as:
\begin{equation}
  f_r(\mathbf{V}_q) = g(\textbf{MLP}([\boldsymbol{\theta}_{f} + \boldsymbol{\theta}_{f,r}; \boldsymbol{\theta}_{l} + \boldsymbol{\theta}_{l,r}]))
\end{equation}
where $\textbf{MLP} : \mathbb{R}^{2d} \to \mathbb{R}^{2d} $ is a multi-layer perceptron network (MLP), $[\cdot;\cdot]$ is concatenation and $g$ is an activate function to generate $\boldsymbol{\theta}_{f}'\in [-L, L]^d, \boldsymbol{\theta}_{l}'\in[0, 1]^d$.
We define $g$ as (Figure~\ref{subfig:projection}):
\begin{equation}
  [g(\mathbf{x})]_i = \begin{cases}
    \boldsymbol{\theta}_{f}'^i\ \ \ \ =L\tanh(x_i), & \text{ if } i\le d, \\
    \boldsymbol{\theta}_{l}'^{i-d}=\sigmoid(x_i),   & \text{ if } i> d.   \\
  \end{cases}
\end{equation}
where $[g(\mathbf{x})]_i$ is the $i$-th element of $g(\mathbf{x})$, $\tanh(\cdot)$ is hyperbolic tangent function and $\sigmoid(\cdot)$ is Sigmoid function.
Note that $\boldsymbol{\theta}_{f}$ as the feature part is flexible to be in $(-\infty, +\infty)$. So in experiments it also works when we remove $\tanh(\cdot)$.
% Besides, to show that feature-logic framework is easy for integration, we can replace MLP with ConvE~\cite{ConvE} to predict transformed query embeddings.
For Experiments please refer to  Section~\ref{sec:exp:analysis}.

\xhdr{Negation Operator $\mathcal{N}$}
The aim of $\mathcal{N}$ is to identify the complement of query set $\llbracket q\rrbracket$ such that $\llbracket \lnot q\rrbracket=\mathcal{V}\backslash \llbracket q\rrbracket$. Suppose that $\mathbf{V}_q=(\boldsymbol{\theta}_{f}, \boldsymbol{\theta}_{l})$ and $\mathbf{V}_{\lnot q}=(\boldsymbol{\theta}_{f}', \boldsymbol{\theta}_{l}')$.
We define the negation operator $\mathcal{N}$ as (Figure~\ref{subfig:complement}):

\begin{equation}
  \begin{aligned}
    \boldsymbol{\theta}_{f}' & = L\tanh (\textbf{MLP}([\boldsymbol{\theta}_{f};\boldsymbol{\theta}_{l}])) \\
    \boldsymbol{\theta}_{l}' & = 1 - \boldsymbol{\theta}_{l}
  \end{aligned}
\end{equation}
where $\textbf{MLP}:\mathbb{R}^{2d} \to \mathbb{R}^{d}$ is a MLP network, $[\cdot;\cdot]$ is concatenation.
The computation of logic part follows NOT operation in vector logic (Eq.~\ref{eq:vector_logic}).

\xhdr{Dyadic Operators}
\label{sec:model:extension}

Benefit from vector logic, our framework is able to directly model all dyadic operators.
We design the same structure for all dyadic operators.
Below we take the Intersection Operator $\mathcal{I}$ and Union Operator $\mathcal{U}$ for example (Figure~\ref{subfig:intersection}~\ref{subfig:union}).
The goal of operator $\mathcal{I}$($\mathcal{U}$) is to represent $\llbracket q\rrbracket = \cap_{i=1}^n \llbracket q_i \rrbracket$ ($\llbracket q\rrbracket = \cup_{i=1}^n \llbracket q_i \rrbracket$).
Suppose that $\mathbf{V}_q=(\boldsymbol{\theta}_{f}, \boldsymbol{\theta}_{l})$ and $\mathbf{V}_{q_i}=(\boldsymbol{\theta}_{q_i,f}, \boldsymbol{\theta}_{q_i,l})$ are feature-logic embeddings for $\llbracket q\rrbracket$ and $\llbracket q_i\rrbracket$, respectively.

First, the feature part outputed from operator is given by the self-attention neural network:
\begin{equation}
  \begin{aligned}
    \boldsymbol{\theta}_{f}' & =\sum_{i=1}^n \boldsymbol{\alpha}_i \boldsymbol{\theta}_{q_i,f} \\
    \boldsymbol{\alpha}_i & = \frac{\exp (\textbf{MLP}([\boldsymbol{\theta}_{q_i,f};\boldsymbol{\theta}_{q_i,l}]))}{\sum_{j=1}^n \exp (\textbf{MLP}([\boldsymbol{\theta}_{q_j,f};\boldsymbol{\theta}_{q_j,l}]))} \\
  \end{aligned}
\end{equation}
where $\boldsymbol{\alpha}_i$ is the attention weight to notice the changes of logic part, $\textbf{MLP}:\mathbb{R}^{2d} \to \mathbb{R}^{d}$ is a MLP network, $[\cdot;\cdot]$ is concatenation.

Second, the logic part of $\mathcal{I}$ ($\mathcal{U}$) should follow AND (OR) operation in vector logic.
Therefore, $\mathcal{I}$ uses $\boldsymbol{\theta}_{l}' = \prod_{i=1}^n \boldsymbol{\theta}_{q_i,l}$  and $\mathcal{U}$ has $\boldsymbol{\theta}_{l}' =\sum_{i=1}^n \boldsymbol{\theta}_{q_i,l}
-\sum_{1\leqslant i < j\leqslant n} \boldsymbol{\theta}_{q_i,l} \boldsymbol{\theta}_{q_j,l}
+\sum_{1\leqslant i < j < k\leqslant n} \boldsymbol{\theta}_{q_i,l} \boldsymbol{\theta}_{q_j,l} \boldsymbol{\theta}_{q_k,l}
+\dotsc +(-1)^{n-1} \prod_{i=1}^n \boldsymbol{\theta}_{q_i,l}$.
% \begin{equation}
%   \begin{aligned}
%     \boldsymbol{\theta}_{l}' =&\prod_{i=1}^n \boldsymbol{\theta}_{q_i,l} \\
%     \boldsymbol{\theta}_{l}' =&\sum_{i=1}^n \boldsymbol{\theta}_{q_i,l}
%     -\sum_{1\leqslant i < j\leqslant n} \boldsymbol{\theta}_{q_i,l} \boldsymbol{\theta}_{q_j,l}
%     +\sum_{1\leqslant i < j < k\leqslant n} \boldsymbol{\theta}_{q_i,l} \boldsymbol{\theta}_{q_j,l} \boldsymbol{\theta}_{q_k,l} \\
%     &+\dotsc +(-1)^{n-1} \prod_{i=1}^n \boldsymbol{\theta}_{q_i,l}
%   \end{aligned}
% \end{equation}
When $n=2$, the logic part is $\boldsymbol{\theta}_{l}' = \boldsymbol{\theta}_{q_1,l}\boldsymbol{\theta}_{q_2,l}$ and $\boldsymbol{\theta}_{l}' =\boldsymbol{\theta}_{q_1,l} + \boldsymbol{\theta}_{q_2,l} - \boldsymbol{\theta}_{q_1,l}\boldsymbol{\theta}_{q_2,l}$, corresponding to the AND and OR operation in vector logic (Eq.~\ref{eq:vector_logic}). The computation complexity is $O(nd)$ where $n$ denotes the number of queries to union and $d$ is the embedding dimension.

Note that the logic part $\boldsymbol{\theta}_{l}'$ only depends on previous logic parts, according to vector logic. The self-attention neural network will learn the hidden information from logic and leverage to the feature part. This architecture makes flexibility come true, which is different from center-size framework.

In fuzzy logic, it is common to use $\min(\cdot)$ and $\max(\cdot)$ as AND and OR operations respectively.
Therefore, we also propose another intersection operator $\mathcal{I}_2$, whose feature part is the same as $\mathcal{I}$ but the logic part is $\boldsymbol{\theta}_{l}' =\min_{i=1}^{n}\{\boldsymbol{\theta}_{q_i,l}\}$.
The other union operator $\mathcal{U}_2$ has $\boldsymbol{\theta}_{l}' =\max_{i=1}^{n}\{\boldsymbol{\theta}_{q_i,l}\}$.

\subsection{Learning Feature-Logic Embeddings}
\label{sec:model:learn_embedding}

We expect the feature-logic embedding of query $q$ and the feature-logic embeddings of entities $v\in \llbracket q\rrbracket$, to achieve high scores.
Relatively, for entities $v'\notin \llbracket q\rrbracket$ and query $q$, we expect low scores.
Therefore, we firstly define a distance function to measure the distance between a given entity embedding and a query embedding, and then we train the model with negative sampling loss.
% Here, the scores are calculated from the neural network output and give the confidence of answers.

\xhdr{Distance Function} Given an entity embedding $\mathbf{v}=(\boldsymbol{\theta}_{v,f}, \boldsymbol{0})$ and a query embedding $\mathbf{V}_q=(\boldsymbol{\theta}_{q,f}, \boldsymbol{\theta}_{q,l})$, we define the conjunctive distance $d_{con}$ between this entity $v$ and the query $q$ as the sum of the feature distance (between feature parts) and the logic part (to expect uncertainty to be 0):

\begin{equation}
  d_{\text{con}}(\mathbf{v};\mathbf{V}_q) = \|\boldsymbol{\theta}_{v,f} - \boldsymbol{\theta}_{q,f}\|_1 +\boldsymbol{\theta}_{q,l}
\end{equation}

For some datasets there exist disjunctive queries in training set, the final distance function $d$ only involves conjunctive distance $(d(\textbf{v};\textbf{V}_{q}) = d_{\text{con}}(\textbf{v};\textbf{V}_{q}))$ as we can train our union operator with disjunctive queries.
However, for cases without disjunctive queries data, because the union operator cannot be trained, we use DNF technique~\cite{BetaE} to transform all queries to DNF.
Given a DNF query $q=q_1\lor \dots\lor q_n$, we define disjunctive distance $d_{\text{dis}}(\textbf{v};\textbf{V}_{q})  =\textbf{OR}\{d_{\text{con}}(\textbf{v};\textbf{V}_{q_1}),\dots,d_{\text{con}}(\textbf{v};\textbf{V}_{q_n})\}$ where $\textbf{OR}$ is OR operation in vector logic (Eq.~\ref{eq:vector_logic}).
% The final distance $d$ is :
The final distance $d$ is based on disjunctive distance $d_{\text{dis}}$ and conjunctive distance $d_{\text{con}}$:
\begin{equation}
  d(\textbf{v},\textbf{V}_{q})       =
  \begin{cases}
    d_{\text{con}}(\textbf{v},\textbf{V}_{q}),\ \text{if }q \text{ is conjunctive}, \\
    d_{\text{dis}}(\textbf{v},\textbf{V}_{q}),\ \text{if }q \text{ is disjunctive}.
  \end{cases}
\end{equation}

\xhdr{Loss Function} Given a training set of queries, we optimize a negative sampling loss
\begin{equation}
  L=-\log\sigma(\gamma-d(\mathbf{v};\mathbf{V}_q))-\frac{1}{k}\sum_{i=1}^k\log\sigma(d(\mathbf{v}'_i;\mathbf{V}_q)-\gamma)
\end{equation}
where $\gamma>0$ is a fixed margin, $v\in\llbracket q\rrbracket$ is a positive entity, $v_i'\notin \llbracket q \rrbracket$ is the $i$-th negative entity, $k$ is the number of negative entities, and $\sigma(\cdot)$ is the sigmoid function.

\subsection{Theoretical Analysis}
\label{sec:model:theoretical_analysis}

We have the following propositions with proofs in Appendix~\ref{sec:appendix:theoretical_analysis}:

\begin{proposition}
  \label{prop:Closure}
  \textbf{Closure}: The projection operators, monadic and dyadic operators are closed under feature-logic embeddings of queries and entities.
\end{proposition}

\begin{proposition}
  \label{prop:Commutativity}
  \textbf{Commutativity}: Given feature-logic embedding $\mathcal{V}_{q_a}, \mathcal{V}_{q_b}$, we have $\mathcal{I}(\mathcal{V}_{q_a}, \mathcal{V}_{q_b}) = \mathcal{I}(\mathcal{V}_{q_b}, \mathcal{V}_{q_a})$ and $\mathcal{U}(\mathcal{V}_{q_a}, \mathcal{V}_{q_b}) = \mathcal{U}(\mathcal{V}_{q_b}, \mathcal{V}_{q_a})$, $\mathcal{I}_2(\mathcal{V}_{q_a}, \mathcal{V}_{q_b}) = \mathcal{I}_2(\mathcal{V}_{q_b}, \mathcal{V}_{q_a})$ and $\mathcal{U}_2(\mathcal{V}_{q_a}, \mathcal{V}_{q_b}) = \mathcal{U}_2(\mathcal{V}_{q_b}, \mathcal{V}_{q_a})$.
\end{proposition}

% \begin{proposition}
%   \label{prop:DeMorgan}
%   \textbf{De Morgan's laws}: Given feature-logic embedding $\mathcal{V}_{q_a}, \mathcal{V}_{q_b}$, we have
%   \begin{equation}
%     \begin{aligned}
%       \mathcal{N}(\mathcal{I}_2(\mathcal{V}_{q_a}, \mathcal{V}_{q_b})) & = \mathcal{U}_2(\mathcal{N}(\mathcal{V}_{q_b}), \mathcal{N}(\mathcal{V}_{q_a})) \\
%       \mathcal{N}(\mathcal{U}_2(\mathcal{V}_{q_a}, \mathcal{V}_{q_b})) & = \mathcal{I}_2(\mathcal{N}(\mathcal{V}_{q_b}), \mathcal{N}(\mathcal{V}_{q_a}))
%     \end{aligned}
%   \end{equation}
% \end{proposition}

\begin{proposition}
  \label{prop:Idempotence}
  \textbf{Idempotence}: Given feature-logic embedding $\mathcal{V}_q$, we have $\mathcal{I}_2(\{\mathcal{V}_q,\mathcal{V}_q,\cdots,\mathcal{V}_q\}) = \mathcal{V}_q$ and $\mathcal{U}_2(\{\mathcal{V}_q,\mathcal{V}_q,\cdots,\mathcal{V}_q\}) = \mathcal{V}_q$.
\end{proposition}

% \begin{proposition}
%   \label{prop:Involution}
%   \textbf{Involution}: Given feature-logic embedding $\mathcal{V}_q$, $\mathcal{V}_q$ is a fixed point of $\mathcal{N}\circ \mathcal{N}$, such that $\mathcal{N}(\mathcal{N}(\mathcal{V}_q)) = \mathcal{V}_q$.
% \end{proposition}

% Proposition~\ref{prop:DeMorgan} illustrates why our framework performs better than previous methods in 2u-DM and up-DM tasks.

% Proposition~\ref{prop:Commutativity}
% All propositions show that our designed  intersection, union and complement operators obey the rules of real logical operations.

The Proposition~\ref{prop:Closure} indicates FLEX is closed. The Propositions~\ref{prop:Commutativity},\ref{prop:Idempotence} show that our designed intersection and union operators obey the rules of real logical operations.


==> paper_section/050_experiment_2cols.tex <==
% In this section, we conduct experiments to demonstrate that: (1) FLEX is a powerful framework for complex knowledge graph reasoning; (2) FLEX is flexible.
% We also conduct extra experi-ments (Section 5.3) to generalise FLEX, since FLEX hasextensibility and flexibility

% Note that experiment results in Section~\ref{sec:exp:result} are based on the simplest implementation of FLEX.
% The results are enough to show that the framework is suitable for complex multi-hop KGR tasks.
% Extra experiments in (Section~\ref{sec:exp:analysis}) of FLEX variants which demonstrate extensibility and flexibility of FLEX are also conducted.
% Extra experiments in (Section~\ref{sec:exp:analysis}) of FLEX variants which demonstrate extensibility and flexibility of FLEX are also conducted.

% we also conduct extended experiments (Section 5.3) to promote FLEX, since FLEX has extensibility
% and flexibility

% Note that experiment results in Section~\ref{sec:exp:result} are based on the simplest implementation of FLEX, whose generalised variants .

% Note that experiment results in Section~\ref{sec:exp:result} are based on the simplest implementation of FLEX, which is inferior to generalised variants in Section~\ref{sec:exp:result}.

% Experiment results in Section~\ref{sec:exp:result} are based on the simplest implementation of FLEX.
% FLEX variants which are more  are shown in \ref{sec:exp:analysis}.

% ## 主要结果

% 总的来说，在无否定和有否定的情况都超过SOTA

% 1. **无否定的情况（表一）：1p 2p 3p 2i 3i pi ip 2u up AVG**
% 2. **有否定的情况（表二）：2in 3in inp pin pni AVG**
% 3. 并查询可以用德摩根公式转换为交+否运算，和真正的集合并不一样。需要给出额外实验说明

% ## 设计的算子和真正集合算子

% 主要是投影和交

% 1. **投影算子** 可以很好地逼近真正的集合投影算子
% 2. **交算子** 可以很好地近似真正的集合交算子
% 3. 模型可以进一步区分空交集，尽管我们并没有在含有空交集的数据集上训练
% 4. 模型可以进一步区分德摩根公式的交运算和真正的集合交运算

% ## 可拓展性

% 拓展1：feature部分可以很复杂，比如有两个：（feature1，feature2，logic）

% 拓展2：logic部分可以选择复数域中的量子逻辑，（feature，quantum logic）

% ## 敏感性分析

% 1. 嵌入维度 [200, 400, 600, 800, 1000]
% 2. 随机种子分别为[1,10,100,1000,10000] 的5次实验得到 error bars

\subsection{Experimental Settings}
\label{sec:exp:setting}

% We adopt the same experimental settings as~\cite{BetaE,ConE}.
% The source code of FLEX is available online~\footnote{\repourl}.

\paragraph{Dataset}
\label{sec:exp:dataset}
We use three datasets in~\cite{BetaE}: FB15k~\cite{Freebase}, FB15k-237 (FB237)~\cite{FB237} and NELL995 (NELL)~\cite{NELL}.
For fair comparison, we use the same query structures in~\cite{BetaE}.
The training and validation queries consist of five conjunctive structures ($1p/2p/3p/2i/3i$) and five structures with negation ($2in/3in/inp/pni/pin$).
We also evaluate the ability of generalization, \ie answering queries with structures that models have never seen during training.
The extra query structures include $ip/pi/2u/up$.
Please refer to Appendix~\ref{sec:appendix:datasets} for more details about datasets.

\paragraph{Training}
\label{sec:exp:train}
We implement our model with PyTorch and use Adam\cite{Adam} as a gradient optimizer.
We use only one GTX1080 graphic card for experiments.
In order to find the best hyperparameters, we use grid search based on the performance on the validation datasets.
Please refer to Appendix~\ref{sec:appendix:train} for best hyperparameters.

\paragraph{Evaluation}
\label{sec:exp:eval}
We adopt the same evaluation protocol as that in \cite{BetaE}. Firstly, we build three KGs: the training KG (training edges), the validation KG (training + validation edges) and the test KG (training + validation + test edges). Given a test query $q$, for each non-trivial answer $v\in \llbracket q\rrbracket_{\text{test}} - \llbracket q\rrbracket_{\text{valid}} $ of the query $q$, we rank it against non-answer entities $\mathcal{V} - \llbracket q\rrbracket_{\text{test}}$. Then we calculate Hits@k (k=1,3,10) and Mean Reciprocal Rank (MRR) based on the rank. Please refer to Appendix~\ref{sec:appendix:eval} for the definition of Hits@k and MRR. For all metrics, the higher, the better.

\paragraph{Baselines}
\label{sec:exp:baselines}

We compare FLEX against four state-of-the-art models, including GQE~\cite{GQE}, Query2Box (Q2B)\cite{Query2box}, BetaE~\cite{BetaE} and ConE~\cite{ConE}.

\subsection{Main Results}
\label{sec:exp:result}
% Note that these experiment results are based on the simplest implementation of FLEX.
% The results are enough to show that the framework is suitable for complex multi-hop KGR tasks.
% We also conduct extra experiments (Section~\ref{sec:exp:analysis}) to generalise FLEX, since FLEX has extensibility and flexibility.
% We compare FLEX against baseline models on queries with and without negation.

\begin{table*}[!t]
  \centering
  % \vspace{1mm}
  \resizebox{0.7\textwidth}{!}{
    \begin{tabular}{c c c c c c c c c c c c c c }
      \toprule
      \textbf{Dataset}       & \textbf{Model} & \textbf{1p}   & \textbf{2p}   & \textbf{3p}   & \textbf{2i}   & \textbf{3i}   & \textbf{pi}   & \textbf{ip}   & \textbf{2u}   & \textbf{up}   & \textbf{AVG}  \\
      \midrule
      \multirow{5}{*}{FB15k} & GQE            & 53.9          & 15.5          & 11.1          & 40.2          & 52.4          & 27.5          & 19.4          & 22.3          & 11.7          & 28.2          \\
                             & Q2B            & 70.5          & 23.0          & 15.1          & 61.2          & 71.8          & 41.8          & 28.7          & 37.7          & 19.0          & 40.1          \\
                             & BetaE          & 65.1          & 25.7          & 24.7          & 55.8          & 66.5          & 43.9          & 28.1          & 40.1          & 25.2          & 41.6          \\
                             & ConE           & 73.3          & 33.8          & 29.2          & 64.4          & 73.7          & 50.9          & 35.7          & \textbf{55.7}          & 31.4          & 49.8          \\
                             & FLEX           & \textbf{77.1} & \textbf{37.4} & \textbf{31.6} & \textbf{66.4} & \textbf{75.2} & \textbf{54.2} & \textbf{42.4} & 52.9 & \textbf{34.3} & \textbf{52.4} \\
      \midrule
      \multirow{5}{*}{FB237} & GQE            & 35.2          & 7.4           & 5.5           & 23.6          & 35.7          & 16.7          & 10.9          & 8.4           & 5.8           & 16.6          \\
                             & Q2B            & 41.3          & 9.9           & 7.2           & 31.1          & 45.4          & 21.9          & 13.3          & 11.9          & 8.1           & 21.1          \\
                             & BetaE          & 39.0          & 10.9          & 10.0          & 28.8          & 42.5          & 22.4          & 12.6          & 12.4          & 9.7           & 20.9          \\
                             & ConE           & 41.8          & 12.8          & 11.0          & 32.6          & 47.3          & 25.5          & 14.0          & 14.5          & 10.8          & 23.4          \\
                             & FLEX           & \textbf{43.6} & \textbf{13.1} & \textbf{11.1} & \textbf{34.9} & \textbf{48.4} & \textbf{27.4} & \textbf{16.1} & \textbf{15.4} & \textbf{11.1} & \textbf{24.6} \\
      \midrule
      \multirow{5}{*}{NELL}  & GQE            & 33.1          & 12.1          & 9.9           & 27.3          & 35.1          & 18.5          & 14.5          & 8.5           & 9.0           & 18.7          \\
                             & Q2B            & 42.7          & 14.5          & 11.7          & 34.7          & 45.8          & 23.2          & 17.4          & 12.0          & 10.7          & 23.6          \\
                             & BetaE          & 53.0          & 13.0          & 11.4          & 37.6          & 47.5          & 24.1          & 14.3          & 12.2          & 8.5           & 24.6          \\
                             & ConE           & 53.1          & 16.1          & 13.9          & 40.0          & \textbf{50.8} & 26.3          & 17.5          & 15.3          & 11.3          & 27.2          \\
                             & FLEX           & \textbf{57.8} & \textbf{16.8} & \textbf{14.7} & \textbf{40.5} & \textbf{50.8} & \textbf{27.3} & \textbf{19.4} & \textbf{15.6} & \textbf{11.6} & \textbf{28.2} \\
      \bottomrule
    \end{tabular}
  }
  \caption{MRR results for answering queries without negation ($\exists$, $\land$, $\lor$) on FB237 and NELL. The results are taken from \citet{ConE}. The best results are in bold. \textbf{AVG} denotes average performance.}
  \label{table:main_results_without_negation}
  % \vspace{-3mm}
\end{table*}

\begin{table*}[!t]
  \centering
  \resizebox{0.50\textwidth}{!}{
    \begin{tabular}{ c c  c c c c  c c c c }
      \toprule
      \textbf{Dataset}       & \textbf{Model} & \textbf{2in}  & \textbf{3in}  & \textbf{inp}  & \textbf{pin}  & \textbf{pni}  & \textbf{AVG}  \\
      \midrule
      \multirow{3}{*}{FB15k} & BetaE          & 14.3          & 14.7          & 11.5          & 6.5           & 12.4          & 11.8          \\
                             & ConE           & 17.9          & 18.7          & 12.5          & 9.8           & 15.1          & 14.8          \\
                             & FLEX           & \textbf{18.0} & \textbf{19.3} & \textbf{14.2} & \textbf{10.1} & \textbf{15.2} & \textbf{15.4} \\
      \midrule
      \multirow{3}{*}{FB237} & BetaE          & 5.1           & 7.9           & 7.4           & 3.6           & 3.4           & 5.4           \\
                             & ConE           & 5.4           & 8.6           & 7.8           & \textbf{4.0}           & \textbf{3.6}           & 5.9           \\
                             & FLEX           & \textbf{5.6}  & \textbf{10.7} & \textbf{8.2}  & \textbf{4.0}  & \textbf{3.6}  & \textbf{6.5}  \\
      \midrule
      \multirow{3}{*}{NELL}  & BetaE          & 5.1           & 7.8           & 10.0          & 3.1           & 3.5           & 5.9           \\
                             & ConE           & 5.7           & 8.1           & 10.8          & 3.5           & 3.9           & 6.4           \\
                             & FLEX           & \textbf{5.8}  & \textbf{9.1}  & \textbf{10.9} & \textbf{3.6}  & \textbf{4.1}  & \textbf{6.7}  \\
      \bottomrule
    \end{tabular}
  }
  \caption{MRR results for answering queries with negation on FB237, and NELL. The results are taken from \citet{ConE}. The best results are in bold. \textbf{AVG} denotes average performance.}
  \label{table:main_results_with_negation}
  % \vspace{-4mm}
\end{table*}

\xhdr{Queries without Negation.} Table~\ref{table:main_results_without_negation} shows the results on queries without negation (EPFO queries).
% Overall, FLEX achieves competitive experimental results within a certain margin of error.
Overall, FLEX outperforms compared models.
FLEX achieves on average 5.2\%, 5.1\% and 3.7\% relative improvement MRR over previous state-of-the-art (SOTA) ConE on FB15k, FB237 and NELL respectively, which demonstrates the advantages of feature-logic framework. % , while 2.6\% relative reduction MRR on FB15k.
Besides, FLEX gains an impressive improvement on queries \textbf{1p}.
For example, FLEX outperforms ConE by 8.9\% for \textbf{1p} query on NELL.
The good results on \textbf{1p} queries enable our further comparison on traditional link prediction tasks with SOTA models, such as TuchER~\cite{TuckER}.
Please refer to Appendix~\ref{LP and MUL}.

\xhdr{Queries with Negation.} Table~\ref{table:main_results_with_negation} shows the results on queries with negation.
Generally speaking, FLEX outperforms BetaE and ConE.
For relative MRR improvement compared with ConE, FLEX achieves 4.1\% on FB15k, 3.4\% on FB237 and 4.7\% on NELL.
The improvement demonstrates the effectiveness of our method.


\subsection{Framework Analysis}
\label{sec:exp:analysis}

\begin{table*}[!t]
  \centering
  \resizebox{\textwidth}{!}{
    \begin{tabular}{l c ccccc ccccc cccc}
      \toprule
      \textbf{Model}       & \textbf{AVG}     & \textbf{1p}      & \textbf{2p}      & \textbf{3p}      & \textbf{2i}      & \textbf{3i}      & \textbf{ip}      & \textbf{pi}      & \textbf{2in}    & \textbf{3in}     & \textbf{inp} & \textbf{pin}    & \textbf{pni}    & \textbf{2u}      & \textbf{up}      \\
      \midrule
      % FLEX                 & 17.6          & 43.2          & 12.6          & 10.8          & 34.3          & 48.0          & 16.3          & 26.3          & 5.2          & 9.2           & 8.1          & 3.9          & \textbf{3.6} & 14.3          & 10.9          \\
      FLEX                 & \underline{18.1} & \textbf{43.6}    & \underline{13.1} & \underline{11.1} & \underline{34.9} & 48.4             & 16.1             & \textbf{27.4}    & 5.6             & \textbf{10.7}    & 8.2          & \underline{4.0} & 3.6             & 15.4             & 11.1             \\
      \midrule
      FLEX-$\infty$        & \underline{18.1} & \underline{43.5} & \underline{13.1} & \underline{11.1} & \underline{34.9} & 48.6             & 16.4             & 26.9             & 5.6             & \underline{10.6} & 8.0          & 3.9             & 3.7             & \underline{15.5} & 11.2             \\
      FLEX-2F              & \textbf{18.3}    & \textbf{43.6}    & \textbf{13.3}    & \textbf{11.2}    & \textbf{35.0}    & \underline{48.8} & \textbf{17.4}    & \underline{27.3} & \textbf{5.8}    & 10.4             & \textbf{8.5} & \textbf{4.1}    & \textbf{4.0}    & \textbf{15.6}    & 11.5             \\
      \midrule
      FLEX-$\mathcal{I}_2$ & 18.0             & 43.3             & 12.8             & 10.9             & 34.8             & \textbf{49.4}    & 15.9             & 27.1             & 5.4             & 9.7              & 8.4          & \textbf{4.1}    & 3.6             & 14.9             & 10.9             \\
      \midrule
      FLEX-$\mathcal{U}$   & \underline{18.1} & 43.3             & 13.0             & \underline{11.1} & 34.5             & 47.7             & 16.6             & 27.0             & \textbf{5.8}    & 10.1             & \textbf{8.5} & \textbf{4.1}    & 3.8             & \textbf{15.6}    & \textbf{11.7}    \\
      % FLEX-$\mathcal{U}_2$ & 18.0             & 43.2             & 12.9             & \underline{11.1} & 34.1             & 48.1             & \underline{16.7} & 27.2             & \underline{5.7} & 10.1             & 8.4          & \textbf{4.1}    & \underline{3.9} & 15.3             & \underline{11.6} \\
      FLEX-1p              & -                & 41.7             & -                & -                & -                & -                & -                & -                & -               & -                & -            & -               & -               & -                & -                \\
      \midrule
      FLEX-w/o-logic & 16.0          & 41.9          & 11.6          & 10.4          & 30.0          & 42.1          & 14.1          & 23.5          & 5.2          & 8.0           & 7.4          & 3.6          & 3.6          & 13.2          & 10.0          \\
      \bottomrule
    \end{tabular}
  }
  \caption{MRR comparison for all variants of FLEX answering queries with \& without negation on FB237. Each variant is based on basic FLEX (first row). The best results are in bold. \textbf{AVG} denotes average performance.
  % From top to bottom, the variants are grouped by feature part modified, logic part modified, training data modified.
  }
  \label{table:variants}
  \vspace{-4mm}
\end{table*}

\begin{figure}
  \centering
  \begin{subfigure}[b]{0.48\columnwidth}
    \includegraphics[width=\columnwidth]{MRR_time.png}
    \caption{MRR and training time.}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.48\columnwidth}
    \includegraphics[width=\columnwidth]{hit_time.png}
    \caption{Hist@10 and training time.}
  \end{subfigure}
  \caption{Impact of dimensionality.}
  \label{fig:impact_of_dim}
  \vspace{-4mm}
\end{figure}

In this section, we conduct extra experiments to analyze FLEX on FB237 dataset.
Table~\ref{table:variants} shows the MRR results of FLEX and its variants on FB237.
% the sensitivity, extensibility and flexibility of feature-logic framework
% \subsubsection{Sensitivity}

\xhdr{Impacts of Dimensionality} Our experiments indicate that the selection of embedding dimension has substantial influence on both effectiveness and efficiency of FLEX.
We train FLEX with embedding dimension $d\in\{200, 400, 600, 800, 1000\}$ and plot results based on the validation set, as shown in Figure~\ref{fig:impact_of_dim}.
With the increase of $d$, the training time rises, while the model performance (indicated by MRR) increases slowly during $d=200$ and $d=800$ but falls after $d=1000$.
Therefore, we decide 800 as the best setting.

\xhdr{Stable Performance} We train and test FLEX five times with different random seeds and report the error bars in Appendix~\ref{sec:appendix:error_bars}. The small standard variances demonstrate the stable performance.

% \subsubsection{Extensibility and Flexibility}
% \label{sec:Extensibility and Flexibility}
% To investigate the extensibility and flexibility of the framework, we compare \textbf{FLEX} with its variants.
% Table~\ref{table:variants} shows the MRR results of \textbf{FLEX} and its variants on FB237.

\xhdr{Extensibility on Feature Part}
(1) Firstly, we show that the feature part can extend to be multiple.
We generate variant FLEX-2F which is FLEX with two feature parts and one logic part. Both feature parts depend on the same logic part, but they do not depend on each other.
Comparing to FLEX, FLEX-2F with two feature parts achieves up to 0.5\% MRR improvement on average, which demonstrates the extensibility of FLEX framework to add more feature parts.
We conclude that more parameters for the feature part result in more accurate reasoning answers, because it contributes to more precise description of entities.
(2) Secondly, we show that the feature part can be extended to be in infinite range.
We generate variant FLEX-$\infty$ which is FLEX with the real space as its feature space, infinite range. Specifically, $\tanh(\cdot)$ is removed in operators.
The result of FLEX-$\infty$ is quite close to FLEX's result on all tasks within 0.003 error.
Therefore, using the real space as the feature space is suitable, which shows the flexibility of the feature part in FLEX.

\xhdr{Flexibility on Logic Part}
We introduce min-based intersection operator and max-based union operator in Section~\ref{sec:model:extension} to show that our logic part is flexible to customize.
So, we generate variant FLEX-$\mathcal{I}_2$ which is FLEX using $\mathcal{I}_2$ as intersection operations.
Both FLEX and FLEX-$\mathcal{I}_2$ achieve similar results on most tasks. Furthermore, FLEX-$\mathcal{I}_2$ gains the best result on $3i$ tasks.
The result demonstrates that different implementations of the logic part slightly affect the final performance.

\xhdr{The Improvement from Closure}
Modeling all closed logical operators allows the framework to train directly on queries with corresponding logical operations, eliminating the need for generalization ability from DNF or De Morgan (DM) formulation.
We design a variant FLEX-$\mathcal{U}$, which is FLEX training on union queries. FLEX-$\mathcal{U}$ uses trainable union operator, instead of DNF or DM, to reason on queries containing union operation. In detail, we append 14968 newly generated \textbf{2u} and \textbf{up} queries to the training set. The validation set and test set remain the same. Note that the generated data doesn't contain any queries in validation set or test set.
From Table~\ref{table:variants}, we observe that FLEX-$\mathcal{U}$ achieves the best performance on \textbf{2u} and \textbf{up}, outperforming FLEX (which uses DNF) by 0.2\% and 0.6\% absolute MRR, respectively.
The result demonstrates that the closure of logical operators is helpful to improve the performance.
% Since generating queries of other logical operations is cheap in real world, we can easily extend the training set to include more queries with different logical operations.
% The result demonstrates that the trainable union operator and specialized union training data contribute to the performance on \textbf{2u} and \textbf{up} tasks.

% is a key to achieve the best performance. It
\xhdr{The Improvement from Logical Data}
The variant FLEX-1p is FLEX trained on \textbf{1p} queries only.
Comparing it with standard FLEX, FLEX-1p achieves the worst performance.
We conclude that extra multi-hop reasoning data is crucial to promote one-hop reasoning.
For more analysis on multi-hop reasoning and one-hop reasoning, please refer to Appendix~\ref{LP and MUL}.

\xhdr{Ablation Study}
(1) If feature part is removed, all entities will be zeros, trivially, according to our definition in Section~\ref{sec:model:component} that the logic part of entity feature-logic embedding is zero.
(2) If the logic part is removed, all logic operators will degenerate into simple neural networks. Then dyadic operators will be attention networks of the same structure, unable to guarantee that they obey the rule of real logical operation.
We design variant FLEX-w/o-logic which removes logic part.
Overall, FLEX-w/o-logic is worse than basic FLEX across all metrics. We conclude that the logic part plays an important role in FLEX.

Because of space limitation, more analysis and experiments are presented in Appendix, including Complexity Analysis~\ref{sec:appendix:complexity_analysis}, Case Study~\ref{sec:appendix:case_study} and More Research Questions~\ref{sec:appendix:more_research_questions}.

% \begin{enumerate}
  % \item \textbf{FLEX-2F}: FLEX with two feature parts and one logic part. Both feature parts depend on the same logic part, but they do not depend on each other.
  % \item \textbf{FLEX-$\infty$}: FLEX with the real space as its feature space, infinite range. Specifically, $\tanh(\cdot)$ is removed in operators.
  % \item \textbf{FLEX-$\mathcal{I}_2$}: FLEX with $\mathcal{I}_2$ as intersection operations (in Section~\ref{sec:model:extension}).
  % \item \textbf{FLEX-$\mathcal{U}$}: FLEX with trainable union operator instead of using DNF or DM. In order to train the union operator, we append 14968 newly generated queries of \textbf{2u} and \textbf{up} structures to the training set. The validation set and test set remain the same. Note that the generated data doesn't contain any queries in validation set or test set.
  % \item \textbf{FLEX-$\mathcal{U}_2$}: FLEX with $\mathcal{I}_2, \mathcal{U}_2$ based on the data setting in \textbf{FLEX-$\mathcal{U}$}.
%   \item \textbf{FLEX-1p}: FLEX with the training data only containing queries of \textbf{1p} structure.
% \end{enumerate}

% Overall, all variants (except \textbf{FLEX-1p}) outperform \textbf{FLEX}. The contributing modifications include more expressive features, more reasonable logic and more training data.
% Note that each variant is based on the simplest \textbf{FLEX}.
% It is said that we may get the best performance result if we apply these contributing modifications in one variant.
% \textbf{FLEX-2F v.s. FLEX.} Comparing to \textbf{FLEX}, \textbf{FLEX-2F} with two feature parts achieves up to 0.5\% MRR improvement on average, which demonstrates the extensibility of FLEX framework to add more feature parts.
% We conclude that more parameters for the feature part result in more accurate reasoning answers, because it contributes to more precise description of entities.

% \textbf{FLEX-$\infty$ v.s. FLEX.} The result of \textbf{FLEX-$\infty$} is quite close to \textbf{FLEX}'s result on all tasks within 0.003 error.
% Therefore, using the real space as the feature space is suitable, which shows the flexibility of the feature part in FLEX.

% \textbf{FLEX-$\mathcal{I}_2$ v.s. FLEX.} We introduce min-based intersection operator and max-based union operator in Section~\ref{sec:model:extension} to show that our logic part is flexible to customize. Both \textbf{FLEX} and \textbf{FLEX-$\mathcal{I}_2$} achieve similar results on most tasks. Furthermore, \textbf{FLEX-$\mathcal{I}_2$} gains the best result on $3i$ tasks. The result demonstrates that different implementations of the logic part slightly affect the final performance.
% The poor performance of \textbf{FLEX-$\mathcal{I}_2$} demonstrates that min-based intersection operator is not necessary in FLEX.

% It achieves the best performance on \textbf{3i} task among all FLEX variants.
% It demonstrates the effectiveness of modified $\mathcal{I}_2$ operator.
% because it gives relatively good results

% \textbf{FLEX-$\mathcal{U}_2$ v.s. FLEX-$\mathcal{I}_2$.} \textbf{FLEX-$\mathcal{U}_2$} significantly outperforms \textbf{FLEX-$\mathcal{I}_2$} on all tasks. We can conclude that we should use both min-based intersection and max-based union.

% \textbf{FLEX-$\mathcal{U}$ v.s. FLEX.} \textbf{FLEX-$\mathcal{U}$} achieves the best performance on \textbf{2u} and \textbf{up}, which demonstrates that the trainable union operator and specialized union training data contribute to the performance on \textbf{2u} and \textbf{up} tasks.
% The favorable results originate from the trainable union operator and specialized union training data.

% \textbf{FLEX-1p v.s. All.} \textbf{FLEX-1p} achieves the worst performance since it has only \textbf{1p} queries for training.
% We conclude that extra multi-hop reasoning data is crucial to promote one-hop reasoning.
% For more analysis on multi-hop reasoning and one-hop reasoning, please refer to Appendix~\ref{LP and MUL}.

% \paragraph{Feature Part Modified}
% \paragraph{Logic Part Modified}
% Flexibility provides the framework with more space to increase its reasoning capability.
% \paragraph{Training Data Modified}


==> paper_section/063_limitation.tex <==
Although the framework is highly extensible, the training time of the framework increases significantly as the number of feature module increases which goes against the concept of environment-friendly and low carbon development.
It is an issue to be explored in the future to make the framework more efficient.


==> paper_section/071_checklist.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
        \answerYes{See Section~\ref{sec:introduction}}
  \item Did you describe the limitations of your work?
        \answerYes{See Section~\ref{sec:appendix:limitation}}
  \item Did you discuss any potential negative societal impacts of your work?
        \answerYes{See Section~\ref{sec:broader_impact}}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
        \answerYes{Yes.}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
        \answerYes{See Section~\ref{sec:model:theoretical_analysis}}
  \item Did you include complete proofs of all theoretical results?
        \answerYes{See Section~\ref{sec:appendix:theoretical_analysis}}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
        \answerYes{See Section~\ref{sec:appendix:train}}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
        \answerYes{See Section~\ref{sec:appendix:datasets}}
  \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
        \answerYes{See Section~\ref{sec:appendix:error_bars}}
  \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
        \answerYes{See Section~\ref{sec:appendix:train}}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
        \answerNA{}
  \item Did you mention the license of the assets?
        \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
        \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
        \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
        \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
        \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
        \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
        \answerNA{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
